Deep Variational Bayes Filters: Unsupervised Learning of State Space Models from Raw Data

We introduce Deep Variational Bayes Filters (DVBF), a new method for unsupervised learning and identification of latent Markovian state space models. Leveraging recent advances in Stochastic Gradient Variational Bayes, DVBF can overcome intractable inference distributions via variational inference. Thus, it can handle highly nonlinear input data with temporal and spatial dependencies such as image sequences without domain knowledge. Our experiments show that enabling backpropagation through transitions enforces state space assumptions and significantly improves information content of the latent embedding. This also enables realistic long-term prediction.

==> computational_architecture.tex <==






\def\interlayer{-2.2cm}%{-1.8cm}
\def\intercolumns{5.5cm}
\def\interboxes{.1cm}
\def\shifty{6.5cm}


\tikzset{>=latex}

\tikzstyle{neuron}=[circle,minimum size=28pt,inner sep=1pt]
\tikzstyle{stochastic neuron}=[rectangle,minimum size=28pt,inner sep=1pt]

\tikzstyle{input neuron}=[neuron,draw=blue!50,fill=blue!25]
\tikzstyle{output neuron}=[neuron,draw=violet!50,fill=violet!25]
\tikzstyle{latent neuron}=[neuron, draw=cyan!75, fill=cyan!25]
\tikzstyle{gen neuron}=[neuron, draw=orange!75, fill=orange!25]
\tikzstyle{recog neuron}=[neuron, draw=teal!75, fill=teal!25]
\tikzstyle{sample neuron}=[stochastic neuron, draw=orange!75, fill=yellow!25]

\tikzstyle{loss node}=[diamond, draw=red, fill=red!25, minimum size = 40pt] 

\tikzstyle{normal edge} = [black, line width=.45mm]
\tikzstyle{dashed edge} = [normal edge, dashed]
\tikzstyle{loss edge} = [red!35, rounded corners, line width = .3mm]
\tikzstyle{sample edge} = [dashed edge, black!35, line width=.3mm]
	   	

\begin{tikzpicture}[->,auto]

% % % % % % % % % % 
% BASIC NODES AND EDGES
% % % % % % % % % %
\foreach \t / \column in {2/1, t-1/2, t/3, t+1/4} {
	\node[input neuron] (inp-\column) at (\column*\intercolumns,\interlayer){$\mathbf{x}_{\t}$};
	
	\node[recog neuron] (rec-\column) at (\column*\intercolumns,2*\interlayer){$\mathbf{h}^{rec}_{\t}$};
	\path (inp-\column) edge[normal edge] (rec-\column);
	
	\node[latent neuron] (lat-\column) at (\column*\intercolumns,3*\interlayer){$\mathbf{y}^{rec}_{\t}$};
	\path (rec-\column) edge[normal edge] (lat-\column);
    
	\node[latent neuron] (prior-\column) at (\column*\intercolumns - 0.3*\intercolumns,3*\interlayer){$\mathbf{y}^{prior}$};
    \node (invisibleKL-\column) at (\column*\intercolumns - 0.15*\intercolumns,3*\interlayer){};
	
	\node[sample neuron] (sam-\column) at (\column*\intercolumns,4*\interlayer){$\mathbf{\tilde{z}}_{\t}$};
	\path 
        (lat-\column) edge[dashed edge] (sam-\column);
        %(prior-\column) edge[sample edge] (sam-\column);
    
    \node[input neuron] (con-\column) at (\column*\intercolumns + 0.3*\intercolumns, 4*\interlayer) {$\mathbf{\bu_{\t}}$};
        
	\node[gen neuron] (gen-\column) at (\column*\intercolumns,5*\interlayer){$\mathbf{z}_{\t}$};
	\path 
        (sam-\column) edge[normal edge] (gen-\column);
	
	\node[output neuron] (out-\column) at (\column*\intercolumns,6*\interlayer){$\mathbf{y}^{gen}_{\t}$};
	\path (gen-\column) edge[normal edge] (out-\column);
}



%\node[input neuron] (con-1) at (1*\intercolumns + 0.5*\intercolumns,4*\interlayer) {$\bu_{t-1}$};


% % % % % % % % % %
% PRIOR
% % % % % % % % % %
%\node[latent neuron] (prior) at (4*\intercolumns, 3*\interlayer){$\mathbf{y}^{prior}$};
%\foreach \column in {1,2,3} {
%	\path (prior) edge[sample edge]  (sam-\column);
%}


% % % % % % % % % %
% LOSSES
% % % % % % % % % %
\node[loss node] (KL) at (4.75*\intercolumns,3.5*\interlayer){KL};
\node[loss node] (NLL) at (5.25*\intercolumns,3.5*\interlayer){NLL};

\path [-, dotted, loss edge, draw=red!25, line width=.5mm] (NLL) -- node [above] { \Huge $ \color{red!50} \mathbf{\oplus}$} (KL);


\node (invisibleNLL-1) at (5*\intercolumns,0.5*\interlayer){};
\node (invisibleNLL-2) at (5*\intercolumns,6.5*\interlayer){};


\foreach \column in {1,2,3,4} {
	\path [loss edge, draw=red!25] (inp-\column) |- (invisibleNLL-1.center) -- (NLL);
	\path [loss edge, draw=red!25] (out-\column) |- (invisibleNLL-2.center) -- (NLL);
    \path 
        [loss edge, draw=red!25] (lat-\column) -- (invisibleKL-\column.center) |- (KL)
        [loss edge, draw=red!25] (prior-\column) -- (invisibleKL-\column.center) |- (KL);
}

%\path [loss edge] (prior) edge (KL);




% % % % % % % % % %
% DOTS
% % % % % % % % % %
\node (dots-tl) at (1.5*\intercolumns, 2*\interlayer){\dots};
\node (dots-bl) at (1.5*\intercolumns, 5*\interlayer){\dots};
\node (dots-tr) at (4.5*\intercolumns, 2*\interlayer){\dots};
\node (dots-br) at (4.5*\intercolumns, 5*\interlayer){\dots};


% % % % % % % % % %
% RECURRENT EDGES
% % % % % % % % % %
\foreach \a/\b in {dots-tl/rec-1, dots-tl/rec-2, rec-2/rec-3, rec-3/rec-4, rec-4/dots-tr} {
    \path
        (\a) edge[normal edge, bend left=10] (\b)
        (\b) edge[normal edge, bend left=10] (\a);
}
\path 


(dots-bl) edge[normal edge] (gen-2)
(gen-1) edge[normal edge] (dots-bl)
(gen-2) edge[normal edge] (gen-3)
(gen-3) edge[normal edge] (gen-4)
(gen-4) edge[normal edge] (dots-br);

% % % % % % % % % %
% INITIALIZATION
% % % % % % % % % %
\node[input neuron] (inp-init1) at (-0.3*\intercolumns, 1*\interlayer){$\xTs$};
\node[input neuron] (inp-init2) at (0.3*\intercolumns, 1*\interlayer){$\uTs$};
\node[recog neuron] (rec-init) at (0*\intercolumns, 2*\interlayer){$\bh_{init}$};
\node[latent neuron] (lat-init) at (0*\intercolumns, 3*\interlayer){$\mathbf{y}_{init}$};
\node[latent neuron] (prior-init) at (-0.3*\intercolumns, 3*\interlayer){$\mathbf{y}^{init}_{prior}$};
\node[sample neuron] (sam-init) at (0*\intercolumns, 4*\interlayer){\innovseed};
\node[gen neuron] (gen-init) at (0*\intercolumns, 5*\interlayer){$\bz_{1}$};
\node[output neuron] (out-init) at (0*\intercolumns, 6*\interlayer) {$\mathbf{y}^{gen}_{1}$};
\node[input neuron] (con-init) at (0.3*\intercolumns, 4*\interlayer){$\bu_{1}$};
\node (invisibleKL-init) at (0*\intercolumns - 0.15*\intercolumns,3*\interlayer){};


\path 
    (sam-init) edge[normal edge] (gen-init)
    (gen-init) edge[normal edge] (out-init)
    (gen-init) edge[normal edge] (gen-1)
    %(prior-init) edge[sample edge] (sam-init)
    (lat-init) edge[dashed edge] (sam-init)
    (rec-init) edge[normal edge] (lat-init)
    (inp-init1) edge[normal edge] (rec-init)
    (inp-init2) edge[normal edge] (rec-init)
    (con-init) edge[normal edge] (gen-1);
    
\path [loss edge, draw=red!25] (inp-init1) |- (invisibleNLL-1.center) -- (NLL);
\path [loss edge, draw=red!25] (out-init) |- (invisibleNLL-2.center) -- (NLL);
\path 
    [loss edge, draw=red!25] (lat-init) -- (invisibleKL-init.center) |- (KL)
    [loss edge, draw=red!25] (prior-init) -- (invisibleKL-init.center) |- (KL);

    
\foreach \first/\second in {init/1, 2/3, 3/4} {
    \path
        (con-\first) edge[normal edge] (gen-\second);
}


% % % % % % % % % %
% DATA
% % % % % % % % % %
\node[rectangle, draw=green, fill=green!25, above of=inp-2, minimum size=28pt, node distance=-\interlayer] (data) {$\mathcal{D}= \left\{\left(\xTs,\uTs\right)_j\mid j=1,\dots,N\right\}$};
 

\foreach \n in {inp-init1, inp-init2, inp-1, inp-2, inp-3, inp-4, con-init, con-1, con-2, con-3, con-4} {
    \node[circle,draw=green, fill=green!25,anchor=south west] at (\n.north east) {\footnotesize $\mathcal{D}$};
}







\end{tikzpicture}

